Vivienne: Relational Verification of Cryptographic Implementations in WebAssembly

This paper explores the use of relational symbolic execution to counter timing side channels in WebAssembly programs. We design and implement Vivienne, an open-source tool to automatically analyze WebAssembly cryptographic libraries for constant-time violations. Our approach features various optimizations that leverage the structure of WebAssembly and automated theorem provers, including support for loops via relational invariants. We evaluate Vivienne on 57 real-world cryptographic implementations, including a previously unverified implementation of the HACL* library in WebAssembly. The results indicate that Vivienne is a practical solution for constant-time analysis of cryptographic libraries in WebAssembly.

==> figs/solving.tex <==
\begin{tikzpicture}[
  scale=1., transform shape,
  tool/.style={font=\normalsize, minimum width = 1cm,
    thick, minimum height = 0.8cm, rounded corners=2pt},
  %% spy using outlines={circle, magnification=5, size=1.5cm, connect spies} %
]
  \node[tool, draw] (sa) {\ac{RelSE}};

  \node[tool, draw, below= 20pt of sa] (z3model) {FS};

  \node[tool, draw, below right = -10pt and 45pt  of z3model, dotted] (z3solve) {Z3.ml Solve};
  %% \node[draw, thick, inner xsep=1em, inner ysep=1em, fit=(z3model) (z3solve),
  %%   label={[fill=white,yshift=-0.3cm]Z3 (ml)}] (z3s) {};

  \node[rounded corners=1pt,
    draw,
    above right = 18pt and 45pt of z3model,
    inner sep = 3pt] (race) {Race};
  \node[rounded corners=2pt,
    inner sep=2pt,
    draw,
    above right = 0.10cm and 0.8cm of race,
    font=\scriptsize] (cvc4) {CVC4};
  \node[rounded corners=2pt,
    inner sep=2pt,
    draw,
    below = 0.1cm of cvc4,
    font=\scriptsize] (z3) {Z3};
  \node[rounded corners=2pt,
    inner sep=2pt,
    draw,
    below = 0.1cm of z3,
    font=\scriptsize] (yices) {yices2};
  \node[rounded corners=2pt,
    inner sep=2pt,
    draw,
    below = 0.1cm of yices,
    font=\scriptsize] (bool) {boolector};

  \draw[->, >={Latex}] (race) -- (cvc4);
  \draw[->, >={Latex}] (race) -- (z3);
  \draw[->, >={Latex}] (race) -- (yices);
  \draw[->, >={Latex}] (race) -- (bool);
  
  \node[draw,
    thick,
    dotted,
    inner xsep=0.2em,
    inner ysep=0.6em,
    fit=(z3) (cvc4) (yices) (bool) (race),
    label={[fill=white,yshift=-0.2cm]Portfolio}] (port) {};
  
  \node[draw,
    thick,
    inner xsep=1em,
    inner ysep=1.5em,
    fit=(sa) (z3model),
    label={[fill=white,yshift=-0.2cm]\toolname}] (box) {};

  \draw [->, >={Latex}] (sa) -- node[left]{$\phi$}(z3model);

  \node[draw, inner xsep=1em, inner ysep=1em, yshift=5pt, fit=(port) (z3solve),
    label={[fill=white,yshift=-0.3cm] SMT Solver}] (z3s) {};


  \draw[->, >={Latex}] (z3model) -- ([xshift=18pt]z3model.east)
  |- node[font=\scriptsize, fill=white, above right=2pt and -4pt]{$n > t$}(race);

  \draw[->, >={Latex}] (z3model) -- node[above]{$\phi'$}([xshift=18pt]z3model.east)
  |- node[font=\scriptsize, fill=white, below right=2pt and -4pt]{$n > t$} (z3solve);


  
\end{tikzpicture}

